Diary matching and the spatial distribution of synthetic travel demand: behavioural representation learning within eqasim

The assignment of daily plans to synthetic individuals largely determines the travel demand used in transport planning and policy evaluation. Matching procedures based on categorical attributes may separate individuals with similar travel behaviour at the boundaries of age or income classes, and agreement at the aggregate level may conceal differences in local demand patterns. We propose Behaviour-Supervised Latent Matching (BSLM), an encoder-decoder approach that learns a 16-dimensional representation of personal, household and residential attributes, supervised by observed travel behaviour. Complete survey diaries are then transferred to synthetic individuals from nearby respondents in this latent space. We compare BSLM with the default Recursive Hot-Deck Matching (RHDM) of eqasim and with an order-independent categorical baseline. In a replay experiment on the Swiss Microcensus, using 37,876 respondents, three donor-exclusion groups and 100 diary draws per person, BSLM reduces the joint-behaviour, ordered-chain and daily-distance scores by 19.5%, 18.5% and 19.4%, respectively, relative to RHDM. We further assign diaries to 850,663 synthetic residents in twenty independent runs. National trip counts are nearly identical across methods, but local purpose patterns differ: shopping trips increase by 0.6% nationally with BSLM compared to RHDM, yet decrease by 5.5% among residents of central Geneva, with larger differences across residential cells. Across twenty random seeds, city-centre mean daily distances by purpose show min-max spans reaching 28.7% of their twenty-run mean. Diary matching should therefore be assessed with individual-level diagnostics and local sensitivity analyses, in addition to aggregate agreement, before its results are used to inform planning decisions.

==> tables/scores.tex <==
\begin{tabular}{lrrr}\toprule
Score (lower is better) & RHDM & BSLM & OHDM \\
\midrule
Energy & 3.341 & 2.690 & 3.284 \\
Chain Brier & 1.211 & 0.987 & 1.193 \\
Distance CRPS (km) & 16.291 & 13.124 & 15.851 \\
Travel-time CRPS (min) & 49.740 & 39.896 & 48.751 \\
Shopping-count CRPS & 0.309 & 0.250 & 0.304 \\
Work-event Brier & 0.150 & 0.110 & 0.147 \\
\bottomrule
\end{tabular}

